Baxos: Backing off for Robust and Efficient Consensus

Leader-based consensus algorithms are vulnerable to liveness and performance downgrade attacks. We explore the possibility of replacing leader election in Multi-Paxos with random exponential backoff (REB), a simpler approach that requires minimum modifications to the two phase Synod Paxos and achieves better resiliency under attacks. We propose Baxos, a new resilient consensus protocol that leverages a random exponential backoff scheme as a replacement for leader election in consensus algorithms. Our backoff scheme addresses the common challenges of random exponential backoff such as scalability and robustness to changing wide area latency. We extensively evaluate Baxos to illustrate its performance and robustness against two liveness and performance downgrade attacks using an implementation running on Amazon EC2 in a wide area network and a combination of a micro benchmark and YCSB-A workload on Redis. Our results show that Baxos offers more robustness to liveness and performance downgrade attacks than leader-based consensus protocols. Baxos outperforms Multi-Paxos and Raft up to 128% in throughput under liveness and performance downgrade attacks under worst case contention scenarios where each replica proposes requests concurrently.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf -f -e '$$pdflatex=q/xelatex %O %S/' $<

fast:
	pdflatex $(FILE)

link:
	ln -s ../$$acm1855741.1855767.bib $$acm1855741.1855767.bib ;

clean:
	for ext in aux log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d

